Spectral Methods for the Complexity of Planar Graph Homomorphisms

We explore the frontier beyond the recently discovered barrier represented by the \emph{quantum automorphism group} $qut(M)$ in the classification theory of planar graph homomorphisms $PlGH(M)$. We show that analyzing the spectral relations of $M$ can prove \#P-hardness when traditional vertex separation and domain-reduction methods with planar edge gadgets provably fail due to the $\qut(M)$ barrier. We prove two criteria of \#P-hardness for $PlGH(M)$: a spectral criterion and a determinant criterion. It is known that the core problem for the classification of $PlGH(M)$ for nonnegative matrices $M$ is for positive definite entry-wise positive matrices. We use the spectral criterion to show that $PlGH(M)$ is \#P-hard for all circulant matrices of prime order $q \ge 3$, while for $q=2$ it is precisely the matchgate case and is P-time computable by the FKT algorithm (for planar perfect matching). We also prove a complexity dichotomy for $\PlGH$ problems defined by tensor products of 2 by 2 matrices. This gives a complete complexity classification for this class of matrices, and the FKT algorithm together with a holographic transformation is \emph{universal}---every $PlGH(M)$ is either (1) P-time computable over all graphs, or (2) \#P-hard in general but P-time computable over planar graphs, or (3) \#P-hard over planar graphs; furthermore, $PlGH(M)$ in (2) consists of precisely those computable by FKT with a holographic transformation.

==> A2.4.Loop_Gadgets.tex <==
\subsection{Loop Gadgets}\label{appendix: loopAppendix}

In this section, we shall explore the loop gadgets,
and gadget interpolation more rigorously.
For $m, n \ge 1$, let
$$\mathcal{P}_{m}(n) = \left\{\mathbf{x} = (x_{i})_{i \in [m]}
\in (\mathbb{Z}_{\geq 0})^{m} \hspace{0.08cm}\Big|\hspace{0.1cm}
\sum_{i \in [m]}x_{i} = n\right\}.$$

We recall that 
$$Z_{M}(\mathbf{L_{n}}G) = 
\sum_{\sigma: V \rightarrow [q]} \prod_{(u, v) \in E}
(M_{\sigma(u)\sigma(u)})^{n} M_{\sigma(u) \sigma(v)}
(M_{\sigma(v) \sigma(v)})^{n} = Z_{\mathbf{L_{n}}(M)}(G),
\quad \text{ for all } n \geq 1,$$
where $\mathbf{L_{n}}(M) = (\diag(M))^{n} \cdot M \cdot (\diag(M))^{n}$.

We can now prove
\cref{lemma: loopLemma}.
The proof is very similar to the proof of
\cref{lemma: thickeningLemma} in
\cref{appendix: thickeningAppendix}.
We first prove the following lemma.

\begin{lemma}\label{lemma: loopLemmaGeneral}
    Let $M \in \Sym{q}{}{\mathbb{R}_{> 0}}$.
    Let $A \in \Sym{q}{}{\mathbb{R}_{\geq 0}}$ be
    a diagonal matrix with positive diagonal entries,  
    that are generated by some $\{g_t\}_{t \in [d]}$,
    such that $A_{ii} = g_{1}^{e_{ii1}} \cdots g_{d}^{e_{iid}}$
    for all $i \in [q]$.
    Furthermore, assume that $e_{iit} \geq 0$ for all
    $i \in [q]$, $t \in [d]$, and that
    $\PlGH(A^{n}MA^{n}) \leq^{T}_{p} \PlGH(M)$ for all $n \geq 1$.
    Then, for any diagonal matrix
    $B \in \Sym{q}{}{\mathbb{R}}$
    of the form
    $$B_{ii} = z_{1}^{e_{ii1}}
    \cdots z_{d}^{e_{iid}},$$
    with parameters
    $\mathbf{z} = (z_{1}, \dots, z_{d}) \in \mathbb{R}^{d}$,
    we have $\PlGH(BMB) \leq^{T}_{p} \PlGH(M)$.
\end{lemma}
\begin{proof}
    We note that
    $$Z_{A^{n}MA^{n}}(G) = 
    \sum_{\sigma: V \rightarrow [q]}
    \left(\prod_{(u, v) \in E} M_{\sigma(u) \sigma(v)} \right)
    \left(\prod_{v \in V}(A_{\sigma(v) \sigma(v)})
    ^{\deg(v) \cdot n} \right),$$
    for all $n \geq 1$.

    We now define the \emph{set}
    $$X(G) = \left\{\prod_{i\in [q]}
    A_{ii}^{k_{i}}\hspace{0.08cm}\Big|\hspace{0.1cm}
    \mathbf{k} = (k_{i})_{i \in [q]} \in
    \mathcal{P}_{q}(2|E|)\right\}, \text{ and }$$
    $$c_{A, M}(G, x) = \sum_{\substack{\sigma: V \rightarrow [q]:\\
    x = \prod_{v}(A_{\sigma(v) \sigma(v)})^{\deg(v)}}}
    \left(\prod_{(u, v) \in E}M_{\sigma(u) \sigma(v)}\right).$$
    We see that
    $$Z_{A^{n}MA^{n}}(G) = 
    \sum_{x \in X(G)} x^{n} \cdot c_{A, M}(G, x).$$
    Crucially, we note that $c_{A, M}(G, x)$ is
    independent of $n$.
    Since $X(G)$ is a set,
    its elements are distinct and 
    $|X(G)| \leq
    |\mathcal{P}_{q}(2|E|)| \leq |E|^{O(1)}$.
    From our assumption that
    $\PlGH(A^{n}MA^{n}) \leq^{T}_{p} \PlGH(M)$,
    oracle access to $\PlGH(M)$
    allows us to compute
    $Z_{A^{n}MA^{n}}(G)$ for
    $n \in [|X(G)|]$.
    This yields a full-rank Vandermonde system,
    which can be solved in polynomial time
    to obtain all $c_{A, M}(G, x)$.

    Next, each $x \in X(G)$ can be written as
    $x = \prod_{i \in [q]}A_{ii}^{k_{i}}$
    for some $\mathbf{k} = (k_{i})_{i \in [q]}
    \in \mathcal{P}_{q}(2|E|)$.
    Since $\{g_t\}_{t \in [d]}$ is a generating
    set of $\{A_{ii}\}_{i \in [q]}$, we note that
    each $x \in X(G)$ admits a unique representation
    $$x = g_{1}^{e_{1}^{x}} \cdots g_{d}^{e_{d}^{x}},
    \qquad e_{t}^{x} = \sum_{i \in [q]}k_{i}e_{iit},$$
    with $e_{t}^{x} \in \mathbb{Z}_{\geq 0}$,
    since all $e_{iit}$, $k_{i} \geq 0$.

    We now define the map
    $\widehat{y}: X(G) \rightarrow \mathbb{R}$ by
    $$\widehat{y}(x) = z_{1}^{e_{1}^{x}} \cdots z_{d}^{e_{d}^{x}},$$
    where $\mathbf{z} = (z_{1}, \dots, z_{d})$ are the parameters
    of $B \in \Sym{q}{}{\mathbb{R}}$.
    Then, for any $\mathbf{k} \in \mathcal{P}_{q}(2|E|)$,
    this definition ensures that
    $$\widehat{y}\left(\prod_{i \in [q]}A_{ii}^{k_{i}}\right)
    = \prod_{i \in [q]}B_{ii}^{k_{i}}.$$
    Now, we define the \emph{set}
    $$Y(G) = \left\{\prod_{i\in [q]}
    B_{ii}^{k_{i}}\hspace{0.08cm}\Big|\hspace{0.1cm}
    \mathbf{k} = (k_{i})_{i \in [q]} \in
    \mathcal{P}_{q}(2|E|)\right\}, \text{ and}$$
    $$c_{B, M}(G, y) = \sum_{\substack{\sigma: V \rightarrow [q]:\\
    y = \prod_{v}(B_{\sigma(v) \sigma(v)})^{\deg(v)}}}
    \left(\prod_{(u, v) \in E}M_{\sigma(u) \sigma(v)}\right).$$

    For any labeling $\sigma: V \rightarrow [q]$, define
    $\mathbf{k}$ such that $k_{i} = 
    \sum_{v \in V: \sigma(v) = i} \deg(v)$.
    Then,
    $$\widehat{y}\left(\prod_{v \in V}
    (A_{\sigma(v) \sigma(v)})^{\deg(v)} \right)
    = \widehat{y} \left(\prod_{i \in [q]}
    A_{ii}^{k_{i}}\right)
    = \prod_{i \in [q]} B_{ii}^{k_{i}}
    = \prod_{v \in V} (B_{\sigma (v) \sigma (v)})^{\deg(v)}.$$
    Hence, for each $y \in Y(G)$,
    $$\left\{ \sigma : V \to [q] \ \middle|\ 
    \prod_{v\in V} (B_{\sigma(v)\sigma(v)})^{\deg(v)} = y \right\}
    = \bigsqcup_{\substack{x \in X(G):\\ \widehat{y}(x)=y}}
    \left\{ \sigma : V \to [q] \ \middle|\ 
    \prod_{v \in V} (A_{\sigma(v)\sigma(v)})^{\deg(v)} = x \right\}.$$
    
    Therefore, we obtain
    $$c_{B, M}(G, y) = \sum_{\substack{x \in X(G):\\
    \widehat{y}(x) = y}} c_{A, M}(G, x).$$
    Using the values of $c_{A, M}(G, x)$ we have already determined,
    we can compute
    $$Z_{BMB}(G) 
    = \sum_{y \in Y(G)}y \cdot c_{B, M}(G, y)
    = \sum_{x \in X(G)} \widehat{y}(x) \cdot c_{A, M}(G, x).$$
    Therefore, $\PlGH(BMB) \leq^{T}_{p} 
    \PlGH(M)$.
\end{proof}

Just as was the case in
\cref{appendix: thickeningAppendix}, we can use
\cref{lemma: loopLemmaGeneral,lemma: MequivalentCM} to prove
\cref{lemma: loopLemma}.

\loopLemma*
\begin{proof}
    We let $A = \diag(M)$ be the diagonal
    matrix with the same diagonal entries as $M$.
    Since the diagonal entries of $A$
    are generated by $\{g_t\}_{t \in [d]}$, we know that
    there exist integers $e_{iit} \in \mathbb{Z}$ s.t.,
    $A_{ii} = g_{1}^{e_{ii1}} \cdots g_{d}^{e_{iid}}$
    for all $i \in [q]$.
    Now, we let $e_{t}^{*} = \min_{i \in [q]}e_{iit}$
    for all $t \in [d]$, and let
    $c = \prod_{t \in [d]}g_{t}^{-e_{t}^{*}}$.
    From \cref{lemma: MequivalentCM}, we see that
    $\PlGH((c A)^{n} M (c A)^{n}) 
    \equiv_p^T \PlGH(A^{n} M A^{n})$.
    Since $\mathbf{L_{n}}(M) = A^{n}MA^{n}$, we know that
    $\PlGH(A^{n}MA^{n}) \leq^{T}_{p} \PlGH(M)$ for all $n \geq 1$.
    So, it follows that $\PlGH((c A)^{n}M(c A)^{n}) \leq^{T}_{p} \PlGH(M)$
    for all $n \geq 1$ as well.
    
    Moreover, we also see that the diagonal entries of the matrix
    $(c A)$ are also generated by
    $\{g_t\}_{t \in [d]}$
    such that $(c A)_{ii} =
    g_{1}^{e_{ii1} - e_{1}^{*}} \cdots g_{d}^{e_{iid} - e_{d}^{*}}$
    for all $i \in [q]$.
    From our choice of $e_{t}^{*}$, it follows that
    $e_{iit} - e_{t}^{*} \geq 0$ for all $i \in [q]$, $t \in [d]$.
    So, \cref{definition: mathcalL,lemma: loopLemmaGeneral}
    imply that $\PlGH(\mathcal{L}(M; \mathbf{z}))
    \leq^{T}_{p} \PlGH(M)$
    for all $\mathbf{z} = (z_{1}, \dots, z_{d}) \in \mathbb{R}^{d}$.
\end{proof}



